Self-supervised Representation Learning with Relative Predictive Coding

This paper introduces Relative Predictive Coding (RPC), a new contrastive representation learning objective that maintains a good balance among training stability, minibatch size sensitivity, and downstream task performance. The key to the success of RPC is two-fold. First, RPC introduces the relative parameters to regularize the objective for boundedness and low variance. Second, RPC contains no logarithm and exponential score functions, which are the main cause of training instability in prior contrastive objectives. We empirically verify the effectiveness of RPC on benchmark vision and speech self-supervised learning tasks. Lastly, we relate RPC with mutual information (MI) estimation, showing RPC can be used to estimate MI with low variance.

==> archive/draft_before_septemper.tex <==
\section{Introduction}
% Learning robust and effective representation has always been the goal of most machine learning paradigms. Supervised learning has been very successful; however, most supervised learning gain a robust representation only by learning from data with hand-specified labels. On the other hand, unsupervised learning has always been a hard task, but well worth exploring because terabytes of unlabeled data are generated each day. Recently, one subfield of unsupervised learning called self-supervised learning has made notable progress \cite{oord2018representation, henaff2019data, chen2020simple}. Self-supervised methods perform particularly well, with the effective group of them are mutual information (MI) based \cite{hjelm2018learning} or MI inspired \cite{oord2018representation}. One major issue of the current MI based methods is the training instability, which we attributes to high variance of losses. Such instability will likely to blow up bias-variance trade-off, cause the model to learn a representation that is far from optimal, or even completely wrong \cite{song2019understanding}. 

% In this paper, we propose relative contrastive learning, a method to improve current MI based representation learning objectives. This method has the following advanrages: 1. 
Modern deep learning networks have achieved great successes in supervised learning[], but labeling data requires immense human labor and inefficient compared to billions of images and text documents online nowadays. Such learning paradigm also prevents application to areas without a large dataset of labeled instances. Unsupervised learning enables a model to learn from unlabeled data, but may not guarantee the learned representation from unlabeled data useful for downstream tasks[], not to mention that the unsupervised fashion can be intrinstically hard and expensive[]. Thus, self-supervised learning has been proposed, where a model automatically generate labels to supervised itself. It doesn't require any label, but can effectively use powerful frameworks designed for supervised learning. Among different designs, contrastive self-supervised learning has gain success. It labels every data in ??. 

However, current constrastive learning is in fact particularly dependent on the choice of learning objective[]. Different objectives result in drastically different performances in downstream tasks like image classification or speech recognition which mostly determines the quality of the learned representation. Many of the current losses have the problem of variance instability[], and small decisions made in hyper-parameters might stop the model from learning meaningful representations by causing the variance to explode[]. Even with small variances, methods like CPC ??.

We introduce a family of objectives called \textit{robust contrastive learning objectives} to improve upon the problems. We measure the contrastive loss by considering four terms: the joint distribution, the square of the joint distribution, the marginal distribution, the square of the marginal distribution, and linearly combine them to serve as the loss for contrastive self-supervised learning. There is no log or exponential term in the loss, thus stabilize the training by avoiding extreme values. This will be later proved by theoretical analysis. Further more, such design allows the model to directly learn without common practices like normalization of hidden embeddings before loss calculation. Our contributions are as follows:

\begin{itemize}
  \item The proposed Chi family losses have strong theoretical guarantees of variance as well as empirical performance on self-supervised learning in visual and audio domain.
  \item We show our losses insensitive to batch size and model architecture, a property current objectives lack.
  \item We can perform adversarial detection in multimodal setting using the proposed losses.
\end{itemize}

\section{Background}
\paragraph{Self-supervised Representation Learning}
Learning robust and effective representation has always been the goal of many machine learning paradigms. Supervised learning has been very successful on many tasks; on the other hand, unsupervised learning has been hard but well worth exploring because terabytes of unlabeled data are generated each day. Self-supervised learning, which predicts a small subset of data using the rest, has made notable progress \cite{oord2018representation, henaff2019data, chen2020simple} due to its superior performance over other unsupervised methods. The basic idea (of self-supervised learning) is to ??. Recent methods \cite{oord2018representation, belghazi2018mine, hjelm2018learning, bachman2019learning} proposed to learn a representation by maximizing of mutual information between latent representations. However, their successes are dependent on choice of contrastive losses~\cite{tschannen2019mutual}, and many losses suffer from large variances~\cite{song2019understanding}. The most commonly used InfoNCE loss from \cite{oord2018representation} has stable variance, but is sensitive to batch size~\cite{song2019understanding, ozair2019wasserstein} and cannot provide a fine-grained (i.e., instance-level, in contrast to population-level) understanding of contrastiveness~\cite{poole2019variational}. Theoretical optimal
% Representation learning aims to extract useful information from raw input (an image or an audio clip) to perform downstream tasks like classification or generation, and usually in a more compact dimension compared to original input (an image represented by a 256 * 256 * 3 matrix to a 1024-dimension vector)~\cite{bengio2013representation}. To learn representation of high quality

\paragraph{Contrastive Representation Learning}
Contrastive learning objectives are widely used in unsupervised representation learning~\cite{arora2019theoretical}, interpretable machine learning~\cite{molnar2019interpretable}, disentangled factor analysis~\cite{hyvarinen2018nonlinear}, and dependency estimation~\cite{hjelm2018learning}. Nonetheless, existing contrastive learning objectives have large variance~\cite{song2019understanding}.

% \paragraph{Mutual information maximization for representation learning}

% Mutual information estimation \cite{belghazi2018mine, hjelm2018learning} has long been used for representation learning, mainly by designing a metric of loss that maximize the lower bound of mutual information between samples and representations \cite{oord2018representation}, or between representations themselves \cite{bachman2019learning}. Estimating mutual information is hard, and recent methods provide tractable gradient-based optimization to estimate \cite{belghazi2018mine}, which makes it suitable to use deep learning architectures. However, \cite{song2019understanding} proves that under some conditions, such estimators will exhibit high variance growing exponentially with the true MI, leading to poor bias-variance trade-off. 

\section{Robust Contrastive Objectives}
We introduce a family of objectives, which we called {\em robust contrastive learning objectives}, that have provable low-variance and admit a point-wise contrastiveness measurement. This new family can be regarded as $\ell_2$ regularized Fenchel's dual program of Pearson $\chi^2$-divergence. 

Our goal is to learn a representation $z = g_{enc}(x)$ given input $x$ that when performing downstream tasks on $x$ we use encoder $g_{enc}$ to extract informative representation $z$. One approach proposed by [] is to maximize the mutual information between $x$ and $y$ which $x$ shares information with. Here $y$ is not a label, but data that is related to $x$. For example,  $x$ and $y$ could be different augmented views of the same image sample, or different patches sampled from the same speech sequence. Note that $x$ and $y$ shares the same objective in the image case or the same speaker and context in the second case. We use $c$ to encode $y$. $z$ and $c$ can use the same or different models.[]

To maximize the mutual information between $x$ and $y$, we use a density function $f(x, y)$ that preserves the mutual information $I(X; Y)$
\begin{equation} \label{eq:def_mi}
    f(x,y) \propto \frac{p(x|y)}{p(x)} \text{   , given   } I(X;Y) = D_{KL}(p(x,y) || p(x)p(y)) = \mathbb{E}_{p(x, y)}\left[\log \frac{p(x | y)}{p(x)}\right]
\end{equation}

We then define our objective function as:
\begin{defn}[$\ell_2$ Regularized Fenchel's Dual Program of Pearson $\chi^2$-divergence]
Denoting $X$ and $Y$ as two random variables, and $x$ and $y$ as their corresponding outcomes, our objective is defined as
\begin{equation*}
    \underset{f \in \mathcal{F}}{\rm sup}\,\,{\rm obj}_f = \,\,\mathbb{E}_{P_{X,Y}}[f(x,y)] - \alpha\, \mathbb{E}_{P_{X}P_{Y}}[f(x,y)] - \frac{\beta}{2}\, \mathbb{E}_{P_{X,Y}}[f^2(x,y)] - \frac{\gamma}{2}\,\mathbb{E}_{P_{X}P_{Y}}[f^2(x,y)],
\end{equation*}
where $\alpha \geq 0$, $\beta \geq 0$, $\gamma > 0$, and $\mathcal{F}$ is any class of functions $f: \mathcal{X} \times \mathcal{Y} \rightarrow \mathbb{R}$ with $\mathcal{X}$ and $\mathcal{Y}$ being the sample spaces .
\label{defn:dual}
\end{defn}
The empirical estimation of our objective (Definition~\ref{defn:dual}) is
\begin{equation}
    \widehat{\rm obj}^{m,n}_f = \mathbb{E}_{P_m}[f(x,y)] - \alpha\, \mathbb{E}_{Q_n}[f(x,y)] - \frac{\beta}{2}\, \mathbb{E}_{P_m}[f^2(x,y)] - \frac{\gamma}{2}\,\mathbb{E}_{Q_n}[f^2(x,y)],
\end{equation}
where $P_m$ and $Q_n$ be the empirical distributions of $m$ i.i.d. samples from the joint distribution $P_{X,Y}$ and $n$ i.i.d. samples from the product of marginal distribution $P_{X}P_{Y}$.

\subsection{Analysis of objective variances}
We provide comparison of variances between the proposed objective and other popular contrastive learning objectives, including Donsker-Varadhan (DV)~\cite{donsker1975asymptotic}; Nguyen, Wainwright,and Jordan (NWJ)~\cite{nguyen2010estimating}; and Contrastive Predictive Coding~\cite{oord2018representation}. Originally these three serves as estimations of $I(X; Y)$, and were adopted to train self-supervised contrastive learning. We use $I_{DV}, I_{NWJ}$ and $I_{CPC}$ to denote them. We have the following lemmas:

\begin{lemm}[Variance of $I_{DV}$]
$\lim_{n\to\infty} n {\rm Var}\Big[\widehat{\rm I_{DV}}^{m,n}\Big] = \Omega \Big(e^{KL(P_m \| Q_n)}-1\Big)$
\end{lemm}

\begin{lemm}[Variance of $I_{NWJ}$]
${\rm Var}\Big[\widehat{\rm I_{NWJ}}^{m,n}\Big] = \Omega \Big((e^{D_{KL}(P_m \| Q_n)}-1) / n\Big)$
\end{lemm}

\begin{lemm}[Variance of $I_{CPC}$]
${\rm Var}\Big[\widehat{\rm I_{CPC}}^{m,n}\Big] = ?$
\end{lemm}

These analysis are based on \cite{song2019understanding}. The variances of $I_{DV}$ and $I_{NWJ}$ are exponential to the KL divergence between the empirical distributions $P_m$ and $Q_n$. This is exactly the ground truth mutual information $I(X;Y)$ because of Equation \ref{eq:def_mi}. $I_{CPC}$ does have low variance, but is sensitive to batch size, since the estimation is saturated by $log(\text{batch size})$.

Before providing the variance analysis of the proposed objectives, we derive the optimal solution

\begin{thm}[Optimal Solution]
The optimal solution for Definition~\ref{defn:dual} is
\begin{equation*}
f^*(x,y) = \frac{p(x,y) - \alpha \, p(x)p(y)}{\beta \, p(x,y) + \gamma \, p(x)p(y)}\,\,{\rm with}\,\, -\frac{\alpha}{\gamma} \leq f^*(x,y) \leq \frac{1}{\beta}.
\end{equation*}
\end{thm}
This is done by taking the functional derivative of Definition 1. The variance of the proposed objective family is the following:

\begin{thm}[Variance of Objective] When $\beta \neq 0$ and $\gamma \neq 0$,$
{\rm Var}\Big[\widehat{\rm obj}^{m,n}\Big] = O\Bigg(\Big( {\rm max}(\frac{\alpha}{\gamma}, \frac{1}{\beta}) \Big)^4 \Bigg)$.
\end{thm}

\textit{Proof}. The optimal solution for Definition 1 

Note that prior contrastive objectives have $\Omega(\frac{e^{I(X;Y)-1}}{n})$\cite{song2019understanding}. This is a huge difference. NCE\cite{oord2018representation} has small variance but requires $\Theta(e^{I(X;Y)})$ as the batch size to have small bias.

\begin{coro}[Relations with Point-wise Mutual Information]
${\rm PMI}(x_1, y_2) \geq {\rm PMI}(x_3, y_4)$ if and only if $f^*(x_1,y_2) \geq f^*(x_3, y_4)$.
\end{coro}
The corollary suggests our optimal solution can be used to estimate point-wise dependency.

\begin{thm}[Consistency]
$\widehat{\rm obj}^{m,n}_f$ is strongly consistent to $$\chi^2_p(P_{X,Y} - \alpha P_XP_Y \,\,\|\,\, \beta P_{X,Y} + \gamma P_XP_Y)=\frac{1}{2}\mathbb{E}_{P_{X,Y}}[\frac{p(x,y) - \alpha \, p(x)p(y)}{\beta \, p(x,y) + \gamma \, p(x)p(y)}] - \frac{\alpha}{2}\mathbb{E}_{P_{X}P_{Y}}[\frac{p(x,y) - \alpha \, p(x)p(y)}{\beta \, p(x,y) + \gamma \, p(x)p(y)}].$$
\end{thm}

\textit{Proof.}

The theorem suggests our objective is a distance between $P_{X,Y} - \alpha P_XP_Y$ and $\beta P_{X,Y} + \gamma P_XP_Y$. Hence, it is a smoothed measurement of dependency between $X$ and $Y$ (a divergence between $P_{X,Y}$ and $P_{X}P_{Y}$). 

\begin{coro}[Fenchel's Dual Program of Pearson $\chi^2$-divergence] Let $\alpha = \beta = 0$ and $\gamma = 1$, our objective recovers Pearson $\chi^2$-divergence between $P_{X,Y}$ and $P_XP_Y$: $\chi^2_p (P_{X,Y}\,\,\|\,\,P_XP_Y)$.
\end{coro}
\begin{coro}[Fenchel's Dual Program of Relative Pearson $\chi^2$-divergence] Let $\alpha = 0$ and $\beta + \gamma = 1$, our objective recovers relative Pearson $\chi^2$-divergence between $P_{X,Y}$ and $P_XP_Y$: $\chi^2_p (P_{X,Y}\,\,\|\,\, \beta P_{X,Y} + \gamma P_XP_Y)$.
\end{coro}

\section{Experiments}
The experiments elaborates the following points. First, our objective maintains low variance in practice, without using techniques like normalization in common practice, which allows our estimation to directly obtain optimal theoretical value of $f$. Then we show our model performs better than other losses in downstream tasks in visual and audio domain. Next, we test our model against different batch size and network designs, and it is the most stable. Lastly, we illustrate how our objective can be used in adversarial sample detection in multimodal setting, a property CPC lacks.

\subsection{Benchmarking Multivariate Gaussian}

\subsection{Robustness to Variance}
Our first experiment is to first demonstrate how variance instability will hurt contrastive learning, then we show the variance stability of the proposed objective. ??How to test variance instability and performance?? 
To show the property of low variance, we provide the training loss in Figure, which equates the negative of the objective itself. Objectives such as DV and NWJ requires normalization to train (in what network and what normalization), otherwise the loss will blow up occasionally during training. CPC does have small variance, but it requires a large batch size in practice. We empirically show that our method doesn't require such normalization to maintain low variance. Such property allows us to directly achieve theoretical optimal by experiments (should be put in the theoretical part), because with normalization or other techniques such as clipping, the empirically estimated density $f$ might not be proportional to the theoretically optimal value. ?? We can say our method preserves contrastive property better than NCE with tricks; and our method preserves relative ratio grows when true ratio grows, and vice versa.

\subsection{Downstream Tasks}
\paragraph{Vision}

We test our proposed objectives in the visual and speech domain. Follow prior works, an encoder network will be trained in a self-supervised fashion without labels. We will then freeze the encoder and train a linear classifier on top using labels to perform on downstream tasks such as image classification in vision and phonetic classification in speech. The image classification results for CIFAR 10 and CIFAR 100 datasets are in Table. Such set up provides (??).
\begin{table}[h!]
\begin{center}
 \begin{tabular}{||c c c||} 
 \hline
 Objectives & CIFAR10 & CIFAR100 \\ 
 \hline\hline
 DV & 91.28 & 0 \\ 
 \hline
 NWJ & 90.54 & 0 \\
 \hline
 NCE & 91.09 & 0 \\
 \hline
 Chi & 91.48 & 0 \\
 \hline
\end{tabular} 
\label{table:img_clf}
\caption{Top-1 accuracy of unsupervised ResNet-18 using linear evaluation.}
\end{center}
\end{table}

\paragraph{Speech}

\subsection{Robustness to Batch Size and Encoder Design}
Methods such as CPC are batch-size-dependent techniques, because the size of negative samples can affect the variances of objectives. We observe from Table that performance our method is much less sensitive to batch size choice especially when batch size is very small, a phenomenon not exhibiting in CPC or other methods. (Describe when batch size is small and large, what is the change; describe the optimal batch size). We conclude that our objective is robust to different batch sizes, especially small batch size. This implies our method can perform effectively well across different hardward conditions.

We then investigate the effect of network choice of the encoder. We train the encoder without label using three networks: a four-layer convolutional neural network, a eighteen-layer ResNet(Res18), and a fifty-layer ResNet(Res50). 

\subsection{Adversarial Multimodal Samples Detection}
Our objective can also effectively detect adversarial samples in a multimodal dataset. Given representations in different modalities for the same object or the same utterance, we can distinguish examples with statistically independent modalities, implying small-to-none connections among modality data for the same sample.
% The experiments serve to 1. demonstrate and quantify how high variance will prevent model from learning optimal representation, 2. show quantitatively how our model can prevent such problem and 3. compare performance among previous methods and our proposed alternative.
% \subsection{Bound variance of mutual information estimation, as well as score function} This is done by providing variance plot of relative MI estimation, as well as the score value
% \subsection{robustness to different mutual information estimations with different variances, especially when the variances are large}
% this is done by running experiments with different classification classes, just like what WPC did for figure 4 number of characters

\begin{thm}[Sample Complexity] 
\end{thm}

\begin{thm}[Consistency]
$\widehat{\rm obj}^{m,n}_f$ is strongly consistent to $$\chi^2_p(P_{X,Y} - \alpha P_XP_Y \,\,\|\,\, \beta P_{X,Y} + \gamma P_XP_Y)=\frac{1}{2}\mathbb{E}_{P_{X,Y}}[\frac{p(x,y) - \alpha \, p(x)p(y)}{\beta \, p(x,y) + \gamma \, p(x)p(y)}] - \frac{\alpha}{2}\mathbb{E}_{P_{X}P_{Y}}[\frac{p(x,y) - \alpha \, p(x)p(y)}{\beta \, p(x,y) + \gamma \, p(x)p(y)}].$$
\end{thm}

\textit{Proof.}

The theorem suggests our objective is a distance between $P_{X,Y} - \alpha P_XP_Y$ and $\beta P_{X,Y} + \gamma P_XP_Y$. Hence, it is a smoothed measurement of dependency between $X$ and $Y$ (a divergence between $P_{X,Y}$ and $P_{X}P_{Y}$). 


==> archive/multicomp.tex <==
Too detailed; how important is for the reviewer to understand the equations. LP needs more details to give comments.

Clarification of self-supervised learning.

Equation -0.5. v1, v2, v2'.

The variance of loss itself from experiments. Variance of our estimator. Bias is the accuracy. 

Previous mutual information high variance: show by experiments measure the variance adopted from previous works.

Multi-modal experiments, show temporal and spatio consistency. Do ASR or other tasks? Harder tasks. Pick tasks that we can improvement.

LP: trying to do one modality really well. Language tasks? Language and vision are better. Speech might be hard.

Amir: the text is written as if it's INCREMENTAL. Generalize to continuous space.

We can study MSE = bias^2 + variance

Torsten: symmetric equation

==> archive/two_page.tex <==
\section{Introduction}
Learning robust and effective representation has always been the goal of most machine learning paradigms. Supervised learning has been very successful on many tasks; on the other hand, unsupervised learning has been hard but well worth exploring because terabytes of unlabeled data are generated each day. Recently, one sub-field of unsupervised learning called self-supervised learning, which predicts a small subset of data using the rest, has made notable progress \cite{oord2018representation, henaff2019data, chen2020simple} due to its superior performance over other unsupervised methods. Many of self-supervised approaches are mutual information (MI) based \cite{hjelm2018learning} or MI inspired \cite{oord2018representation}. Mutual information measures statistical divergence between random variables by measuring Kullback–Leibler (KL) divergence from joint distribution to product of marginal distributions. One major issue of the current MI based methods is the training instability, which we attributes to high variance of losses. Such instability will sometimes blow up bias-variance trade-off, cause the model to learn a representation that is far from optimal, or one that is even completely wrong \cite{song2019understanding}. 
% . We thus replace KL divergence with Pearson divergence for better numerical stability, and further use relative ratio to bound variance of estimation and stabilize training. We prove, in theory and in practice, that such stability will help current models learn a better representation, have superior convergence rate, and achieve much better results. 


In this paper, we proposed Relative Chi-Squared Dependency Coding, which uses Pearson Chi-Square divergence \cite{pearson1900x} to estimate square mutual information \cite{sugiyama2013machine}, and bounds the variance of estimation by using relative density ratio \cite{yamada2013relative}. In theory, the proposed method are bounded by an error term proportional to the inverse of sample size. In practice, we show our approach reduces the instability during training, exhibits higher convergence rate, and leads to higher than state-of-the-art results on different representation learning tasks.

\section{Chi-Squared Relative Dependency Coding}
% \subsection{Mutual Information Estimation for Representation Learning}
% Mutual information estimation \cite{belghazi2018mine, hjelm2018learning} has long been used for representation learning, mainly by designing a metric of loss that maximize the lower bound of mutual information between samples and representations \cite{oord2018representation}, or between representations themselves \cite{bachman2019learning}. Estimating mutual information is hard, and recent methods provide tractable gradient-based optimization to estimate \cite{belghazi2018mine}, which makes it suitable to use deep learning architectures. However, \cite{song2019understanding} proves that under some conditions, such estimators will exhibit high variance growing exponentially with the true MI, leading to poor bias-variance trade-off. 
\subsection{Squared Mutual Information}
Current mutual information based representation learning models suffer from high variance. To balance bias and variance, we seek for objectives that are more stable. Recently an alternative to MI, Square Mutual Information (SMI), was introduced to approximate divergence numerically more stable than traditional MI. Mutual information for two random variables, (equation), is the KL divergence from joint distribution of two random variables to the product of marginal distributions. 
\[MI(x, y) = \int\int_{} p(x, y)log\frac{p(x, y)}{p(x)p(y)}dxdy\]
SMI, on the other hand, replaces KL divergence with Person Chi-Squared divergence. 
\[SMI(x, y) = \frac{1}{2} \int\int_{} p(x)p(y)(\frac{p(x, y)}{p(x)p(y)} - 1)dxdy\]
SMI was proved to achieve optimal non-parametric convergence rate, it has superior numerical properties, and it is robust against outliers \cite{sugiyama2013machine}.

\subsection{Relative Density-Ratio Estimation}
To estimate SMI, \cite{kanamori2009least} proposed to accurately estimate SMI based on density-ratio approximation. However, \cite{yamada2013relative} pointed out under some conditions \cite{kanamori2009least} will diverge to infinity thus unreliable, and proposed an alternative approach named relative density ratio estimation. We adopt this method in this paper, due to the fact that it bounds variance by an error term of $\frac{1}{n}$ where $n$ is the sample size and variance is independent of model complexity, both beneficial to learning. 

\subsection{$\chi^2$ Relative-Dependency Coding for Representation Learning}

Assuming $v_1$/$v_2$ are two different views for the same data and $v_2'$ is a view for another data, $F$/$G$ being two mapping functions, we propose the following {\em $\chi^2$ Relative-Dependency Coding} ($\chi^2$R-DC)
:
{\small
\[\max _{F,G}\,\max _{\hat{r}_{\theta}}\, \mathbb{E}_{P_{\mathcal{V}_1, \mathcal{V}_2}}\left[\hat{r}_{\theta}(F(v_1), G(v_2))\right]-\frac{\alpha}{2} \mathbb{E}_{P_{\mathcal{V}_1, \mathcal{V}_2}}\left[\hat{r}^{2}_{\theta}(F(v_1), G(v_2))\right]-\frac{1-\alpha}{2} \mathbb{E}_{P_{\mathcal{V}_1},P_{\mathcal{V}_2}}\left[\hat{r}^{2}_{\theta}(F(v_1), G(v_2'))\right]-\frac{1}{2}\]}
with $\hat{r}_{\theta}$ being the output of a score function pre-defined encoder (ResNet, LSTM, etc) plus a score function. $\alpha$ is the density ratio which can determine the bound of variance, and $F(\cdot)$ and $G(\cdot)$ represent encoded representation. We show that $\chi^2$R-DC aims at learning $F$/$G$ so that the statistical dependency between the learned representations from the correlated views are maximized (proof ignored).

\section{Experiments}
The experiments serve to 1. demonstrate and quantify how high variance will prevent model from learning optimal representation, 2. show quantitatively how our model can prevent such problem and 3. compare performance among previous methods and our proposed alternative.
\subsection{Audio}
We pre-train the proposed objective on LibriSpeech \cite{panayotov2015librispeech} dataset and we consider the 100h and 360h splits of clean data. Then we use the pre-trained model on downstream tasks like phoneme classification.

\subsection{Image}
We apply our objective on AMDIM \cite{bachman2019learning}, a publicly available mutual information based model that achieved comparable results to state-of-the-art on self-supervised object recognition. We evaluate the quality of the representation of our objective by using a linear or multilayer perceptron classifier on top our learned representation, a standard practice among literature. The results are in table 1.
\begin{table}
\centering
\begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|  }
 \hline
 \multicolumn{3}{|c|}{Results of different objectives (linear / MLP)} \\
 \hline
 Loss & CIFAR 10 & CIFAR 100 \\
 \hline
 NCE\cite{oord2018representation}   & 93.1, 91.2    &72.8, 70.2 \\
%  JS & - & - \\
%  WPD\cite{ozair2019wasserstein} & - & - \\
 $\chi^2$R-DC &92.4, 91.3  & 72.1, 69.7\\
 \hline
\end{tabular}
\caption{Initial results for different losses on AMDIM}
% \label{table:table1}
\end{table}

In the future we will design experiments that shows: 1. Our objective is more stable than others; 2. Our objective has better convergence rate than others; 3. The variance of our objective is bounded and independent of model complexity. We will also apply our objective on another close to state-of-the-art model CMC \cite{tian2019contrastive} to further prove that our loss have the properties we claim across different designs of unsupervised learning architecture.

\section{Questions}
What kind of the suggestion you will made on the presentation/experimental design? Does STOA results which performs better than previous losses necessary?
Is the presentation approachable overall?

==> sections/0_abstract_archive.tex <==
Among different self-supervised learning objectives, contrastive learning methods are the most popular ones due to its strong empirical performance. 
These methods often use objective functions that maximize the discrepancy between the distribution of related samples and a noise distribution. 

introduce a practical objective with lower variance and less sensitivity to minibatch size. The objective does not contain any exponential or logarithm terms that some objectives have; it also measures the averaged effect, instead of picking one sample from many samples like Contrastive Predictive Coding \citep{oord2018representation} does. We show that our proposed objective outperforms other objectives on self-supervised learning for both vision and speech tasks.

We propose a family of objectives based on Pearson Chi-Square divergence for self-supervised learning using contrastive loss. The new objectives tackles variance instability common in contrastive training, a problem which fatalistically affects quality of the learned representation from self-supervised learning. We design the loss by measuring $\Chi^2$ divergence between the joint probability and the marginal probability of two representations of the same object, plus two regularizing terms derived from the $\Chi^2$ divergence between the marginal and the joint. Such design allows us to theoretically upper bound the variance of objectives, and empirically provide stable loss. The proposed method shows highly competitive performance in downstream classification tasks in visual and audio domain, insensitiveness to architecture or batch size, and ability to perform adversarial detection in a multimodal dataset (like Visual Question Answering, ?, ). The systematic theoretical analysis and strong empirical performance demonstrate that the new objective effectively reduce variance and thus provide higher quality representation after self-supervised training.
We replace Kullback–Leibler (KL) divergence with Pearson Chi-Square divergence and apply relative ratio estimation to solve stability and robustness problem among mutual information based representation learning models. Mutual information measures statistical divergence between random variables by measuring KL divergence from joint distribution to product of marginal distributions. Recently many methods design learning objectives either by maximizing lower bound of mutual information, a ratio proportional to mutual information, or other metrics similar to mutual information. These settings particularly suit self-supervised learning, a branch of unsupervised learning which aims to predict a small subset of data using the rest, and has achieved significant improvement over other unsupervised learning designs. However, most of these methods are quite unstable, making it hard for real-world models to apply and harness the power of unlabeled data. We thus replace KL divergence with Pearson divergence for better numerical stability, and further use relative ratio to bound variance of estimation and stabilize training. We prove, in theory and in practice, that such stability will help current models learn a better representation, have superior convergence rate, and achieve much better results. 

==> sections/1_intro_archive.tex <==
is inspired by the relative discrepancy estimation \citep{yamada2013relative}. Compared to an ordinary discrepancy which estimates difference of two distributions, relative discrepancy estimates difference of a distribution and a mixture of two distributions, and has constrained density ratio \citep{sugiyama2012density} and lower variance \citep{yamada2013relative}. 

Original
Unsupervised representation learning has drawn tremendous attention in the machine learning community over the last few years because of its power to extract good representation given no supervision of manually specified labels. Self-supervised learning, a subset of unsupervised learning, has outstanding performance on representation learning by obtaining pseudolabels from the data itself \citep{liu2020self}. Among its mainstream strategies, contrastive self-supervised learning has been proved successful on tasks including visual object recognition \citep{he2020momentum, tian2019contrastive, chen2020big}, speech recognition \citep{oord2018representation, riviere2020unsupervised}, language modeling \citep{kong2019mutual}, graph representation learning \citep{velickovic2019deep} and reinforcement learning \citep{kipf2019contrastive}. The idea of self-supervised contrastive learning is to learn latent representations such that semantically similar instances (or defined as \textit{positive} samples) will have closer representations, while dissimilar instances (or defined as \textit{negative} samples) will have distant representations \citep{arora2019theoretical}. 

To contrast representations of similar and dissimilar instances, prior work has formulated the contrastive learning objectives as maximizing the discrepancy between the distribution of similar instances and the distribution of dissimilar instances. For instance, the Kullback–Leibler (KL) divergence between distributions such as Donsker-Varadhan bound (DV; \citealp{donsker1975asymptotic}), Nguyen-Wainright-Jordan bound (NWJ; \citealp{nguyen2010estimating}) and Contrastive Predictive Coding (CPC; \citealp{oord2018representation}), the Jenson-Shannon divergence such as JSD bound \citep{nowozin2016f}, and Wasserstein divergence such as Wasserstein Predictive Coding (WPC; \citealp{ozair2019wasserstein}). Although the choices of objectives are abundant, three main challenges that can hardly be well addressed at the same time: training stability, sensitivity to minibatch size, and downstream performance. For example, DV and NWJ suffer from large variances which destabilize training and cause suboptimal performance \citep{poole2019variational, hjelm2018learning, tschannen2019mutual}. CPC achieves good performances on downstream tasks \citep{oord2018representation}, but its downstream performances are more sensitive to minibatch size \citep{poole2019variational, ozair2019wasserstein}.



%%%%%%%%%%%%%%%%%%Important
because of two reasons: CPC itself is upper bounded by the logarithm of the minibatch size, and will learn better representation by distinguishing one positive sample from many negative samples when the pool of negative samples is larger \citep{ozair2019wasserstein}. 

will force the model to have better discriminative power by distinguishing one positive sample from many negative samples when the pool of negative samples is larger \citep{ozair2019wasserstein}.

** dont' say our method solves these problmes. Be soft. we attempt to solve. 


[Unlike CPC, which selects one sample out of many samples in the same minibatch, we compute the averaged effect over groups of samples,  thus is less dependent on minibatch size compared to CPC \citep{oord2018representation, ozair2019wasserstein}.]

In essence, we employ the Pearson Chi-Square divergence instead of the KL divergence as a training objective. Also, we estimate a bounded \textit{relative} density ratio to replace the unbounded density ratio in other methods to overcome the high variance. As a result, RPC does not include any logarithmic or exponential term, and maintains lower variance than DV, NWJ and JSD whose large variances will destabilize training and cause worse performance \citep{poole2019variational, hjelm2018learning, tschannen2019mutual}.  Unlike CPC, which selects one sample out of many samples in the same minibatch, we compute the averaged effect over groups of samples,  thus is less dependent on minibatch size compared to CPC \citep{oord2018representation, ozair2019wasserstein}. 


To conclude, RPC not only outperforms other methods on different downstream tasks, but also exhibits lower variance and has less sensitivity during training. 

RPC is inspired by the {\em relative} discrepancy between the joint and product of marginal distribution under Pearson Chi-square divergence. RPC enjoys [how the three challenges could be balanced] two major advantages: {\em better training stability} and {\em less batch-size sensitivity}. 

However, many of these objectives exhibit large variances, which will destabilize training due to numerical issue \citep{poole2019variational, hjelm2018learning, tschannen2019mutual}, or result in a lower downstream task performance \citep{tschannen2019mutual, tsai2020neural}. The reasons for large variances are two-folds: first, the objectives often have logarithm or exponential terms; second, (the ratio $p_{xy} / p_xp_y$ is unconstrained).


To bound the ratio, we use relative ratio. To reduce the training variance, we use a loss without any logarithm or exponential terms. As a result the variance of the objective has an asymptotic variance bound. Compare to CPC and WPC, which is instance-wise method, we are group-wise method and is less sensitive to batch size. Most importantly, our objective outperforms other objectives on downstream tasks in both vision and speech domain.

DV and NWJ are based on the Kullback–Leibler divergence, and JSD is based on the Jensen–Shannon divergence. CPC and WPC do not \colorbox{red}{help needed from Hubert} (CPC and WPC is not exactly dependency based, but they are based on KL and Wasserstein.)
 
Representation learning has drawn tremendous attention in machine learning community over the last few years, because of its power to entangle different explanatory factors of variations behind the data~\citep{bengio2013representation}. In supervised learning, effective representations can be learned directly through manually specified labels. However, generating labels is both expensive and difficult, and hence many unsupervised learning methods are proposed. Among mainstream unsupervised learning strategies, self-supervised learning is a class of discriminative unsupervised learning algorithms that are given supervision not by manual labels but by the model itself. It has been able to learn effective representations for object recognition in computer vision \citep{he2020momentum, tian2019contrastive, chen2020big}, speech recognition in speech processing \citep{oord2018representation, riviere2020unsupervised}, language modeling in natural langauge processing \citep{wu2019self}, graph representation learning \citep{velickovic2019deep} and state transition predictions in reinforcement learning \citep{kipf2019contrastive}. 
Different loss design, given exactly the same automatic labeling techniques, will result in drastically distinct representations. Therefore, it is of vital importance to design proper objective functions for contrastive learning to take advantage of these instances. 

. representation learning will be a challenging task under unsupervised learning settings, as it will lack labeled responses or human supervisions

Learning effective representations has been one of the central tasks of machine learning. Among mainstream paradigms, unsupervised methods need to effectively create learning signals without labeled responses or human supervisions. Considering the nature that many downstream tasks are discriminative, a discriminative unsupervised method is efficient as it learns representation without generating data. Recently, self-supervised learning, a class of discriminative unsupervised learning algorithms that automatically generate labels not by human but by models, has been able to learn effective representation for object recognition in computer vision, speech recognition in speech processing, and state transition predictions in reinforcement learning. A large portion of these successful methods automatically generate labels in a contrastive manner, which basically group the unlabeled input to related pairs (termed \textit{positive pairs}) and unrelated pairs (termed \textit{negative pairs}), and assign different labels to the positive and negative groups. 


Contrastive learning has been proved successful in self-supervised learning \citep{henaff2019data, tian2019contrastive}. The idea is to learn representations so that semantically similar instances will have close representations, while dissimilar ones will have distant representations in the embedding space. Recent literature has related the success of contrastive self-supervised learning to objectives based on dependency estimation methods, such as Donsker-Varadhan (DV; \citet{donsker1975asymptotic}), Nguyen-Wainright-Jordan (NWJ; \citet{nguyen2010estimating}), Jenson-Shannon Divergence (JSD; \citet{hjelm2018learning}), Contrastive Predictive Coding (CPC; \citet{oord2018representation}) and Wasserstein Predictive Coding (WPC; \citet{ozair2019wasserstein}). DV and NWJ are based on the Kullback–Leibler divergence, and JSD is based on the Jensen–Shannon divergence. CPC and WPC do not \colorbox{red}{help needed from Hubert} (CPC and WPC is not exactly dependency based, but they are based on KL and Wasserstein.)

However, theoretical and empirical evidences show drawbacks of these objectives. DV and NWJ may exhibit high variance \citep{song2019understanding} that could disrupt the training \citep{poole2019variational, hjelm2018learning} or lower downstream performance \citep{tschannen2019mutual}. CPC needs to include a sufficient amount of examples in one batch to have a low bias \citep{song2019understanding, poole2019variational}, thus empirically needs a batch of enough samples to learn a good representation \citep{ozair2019wasserstein}. WPC and JSD show worse empirical performance than CPC \colorbox{red}{Citation here} in some representation tasks. 

In this paper, we introduce a novel, parameterized, and dependency based contrastive objective, the Robust Contrastive Objective (RCO) for self-supervised representation learning. It obtains a level of lower variance and robustness to batch size differences. It does not have logarithmic or exponential terms which other objectives have. Empirically it exhibits lower variance during training and better downstream performance than DV and NWJ. In terms of batch size, CPC and WPC aim to distinguish a positive sample away from many negative samples in a batch, so a larger batch size will construct more negative samples, and better representation will be obtained as the task will be more non-trivial. On the other hand, RCO objective directly maximizes the divergence between positive samples distributions and the negative sample distributions, by computing the expectation statistics. Number of negative samples does not have a direct impact on the difficulty of the task, and thus RCO is less sensitive to batch size. 

a larger number of negative samples will not likely The task will be non-trivialNumber of negative samples will influence RCO less, 
RCO does not include any logarithmic or exponential term and only consists of up to a squared term, which asymptotically bound its variance. 

We will illustrate the following in this paper: 
\begin{itemize}
  \item RCO has strong performance on downstream tasks, including both vision and speech representation learning.
  \item Theoretical analysis and empirical demonstration of the variance behavior.
  \item Performance comparison under small batch sizes between RCO and CPC.
\end{itemize}
Effects of the parameters in the objective, ablation study of other components in the training, and relation to mutual information estimation will also be shown in the later part of the paper.

==> sections/2_method_arxiv.tex <==
\subsection{========================}

Given two probability measures, $P$ on sample space $\mathcal{X}$ and $Q$ on sample space $\mathcal{Y}$, we define a scoring function $f$ represented by a neural network with parameters $\theta$, that maps from \colorbox{yellow}{$\mathcal{X} \times \mathcal{Y}$} to a single scalar. The Relative Predictive Coding maximizes the following discrepancy between $P$ and $Q$:

where $\alpha\geq 0, \beta\geq 0$ and $\gamma\geq 0$ are predefined hyperparameters we call \textit{relative parameters} to regularize $f$. To estimate Equation \ref{eq:RPC_math_def}, we draw samples from $P$ and $Q$.  Let $\hat{P}_m$ denote the empirical distribution of $m$ i.i.d. samples from $P$ and $\hat{Q}_n$ denote the empirical distribution of $n$ i.i.d. samples from $Q$. $\mathbb{E}_{\hat{P}_m}$ and $\mathbb{E}_{\hat{Q}_n}$ denote the sample averages over $\hat{P}_m$ and $\hat{Q}_n$ respectively. The empirical estimator $\hat{I}_{\mathrm{RPC}}$ is 
\begin{equation} \label{eq:RPC_empirical_def}
\hat{I}_{\mathrm{RPC}}^{m, n}=\mathbb{E}_{\hat{P}_{m}}[f_{\theta}]-\alpha \mathbb{E}_{\hat{Q}_{n}}[f_{\theta}]-\frac{\beta}{2} \mathbb{E}_{\hat{P}_{m}}\left[f_{\theta}^{2}\right]-\frac{\gamma}{2}\mathbb{E}_{\hat{Q}_{n}}\left[f_{\theta}^{2}\right].
\end{equation}

In practice, given a minibatch of samples, we start from the viewpoint of a single sample. The empirical distribution $\hat{P}_m$ is formed by drawing samples that are related to the single sample (i.e., positive samples), and $\hat{Q}_n$ draws samples unrelated to the single sample (i.e., negative samples). We estimate $\hat{I}_{\mathrm{RPC}}^{m, n}$ with respect to every training sample in the minibatch, and then average them for final loss calculation. 

After introducing the objective, we will investigate a problem that DV, NWJ and JSD exhibit: the high variance. Compared to them, whose estimations contain exponentiation or logarithm of $f$, Relative Predictive Coding only has linear and quadratic terms. In fact, we are able to provide an asymptotically result for the variance of $\hat{I}_{\mathrm{RPC}}^{m, n}$ :


We defer the proof to \colorbox{yellow}{Appendix}. \colorbox{yellow}{$\beta \leq 1 ?$}From Proposition \label{prop:variance}, the variance of $\hat{I}_{\mathrm{RPC}}^{m, n}$ is asymptotically bounded by the $({\rm max}(\frac{\alpha}{\gamma}, \frac{1}{\beta}) )^4$, which is further multiplied by $(\frac{\beta^2}{4m}+\frac{\gamma^2}{4n})$, a term much smaller than 1.0 in practice. Empirically we observe a much smaller variance than the bound. In contrast, \citet{song2019understanding} shows that $\lim _{n \rightarrow \infty} n \Var[\hat{I}_{\mathrm{DV}}^{m, n}] \geq (e^{D_{\mathrm{KL}}(P \| Q)}-1)$ and ${\Var}[\hat{I}_{\mathrm{NWJ}}^{m, n}] \geq ((e^{D_{\mathrm{KL}}(P \| Q)}-1) / n)$. The lower bounds of $\Var[\hat{I}_{\mathrm{DV}}^{m, n}]$ and $\Var[\hat{I}_{\mathrm{NWJ}}^{m, n}]$ could grow exponentially with the true $\KL(P \Vert Q)$, which is often unknown and large in real-world scenarios \citep{rhodes2020telescoping}, while the upper bound of $\Var[\hat{I}_{\mathrm{RPC}}^{m, n}]$ could be parameterized and independent of $\chi^2(P \Vert Q)$. Our objective suggests a more appealing alternative in terms of variance stability.
\begin{wrapfigure}{r}{0.3\textwidth}
  \begin{center}
    \includegraphics[width=0.28\textwidth]{fig/r_beta.png}
  \end{center}
  \caption{Illustration showing that the parameter $\beta$ in relative density ratio $r_{\beta} = p / (\beta p + (1 - \beta) q)$ (e.g., $\beta =0.5, 0.95$) has successfully bounded the unconstrained density ratio $r = p / q$ (i.e., $\beta=0$).}
  \label{fig:relative}
\end{wrapfigure}

The RPC is also less sensitive to minibatch size changes. Compared to CPC, which is upper bounded by logarithm of minibatch size, RPC itself is not bounded by any function of the minibatch size. More importantly, CPC tries to score the single positive sample relatively \textit{higher} than the negative samples. Since from the viewpoint of every data point, there will be only one positive sample in a minibatch, pushing score of one sample higher than scores of other samples would be relatively easy if there are insufficient samples to give scores to. In contrast, RPC pushes the averaged score for positive samples high \textit{and} the averaged scores for negative samples low simultaneously to maximize the objective. Even when the minibatch size is small, RPC aims for a high score for every positive sample and a low score for negative samples, where the minibatch size insensitivity comes from. 

% Our objective is also closely related to Chi-square divergence. The \textit{$\chi^2$-divergence} $(\chi^2)$ is a member of the $\textit{f}$-divergences that not only shares similar properties \citep{niu2013squared} with the KL divergence, but also has superior numerical properties \citep{kanamori2013computational} and robustness against outliers \citep{sugiyama2012density}. , and it has been used in semi-supervised representation learning \citep{niu2013squared}. The special cases of our objective would recover $\chi^2_p$ and its form that estimates the relative density $P / (\beta P + (1 - \beta) Q)$ ~\citep{yamada2013relative}:

Our objective is also closely related to Relative Chi-square divergence \citep{yamada2013relative}. The Chi-square divergence between two distributions $P$ and $Q$ is defined as $\chi^2(P \Vert Q) = \frac{1}{2} \mathbb{E}_Q[(r - 1)^2]$, where $r = p / q$ is called \textit{density ratio}, with $p$ and $q$ being probability densities of $P$ and $Q$ respectively. Because the unbounded density ratio $r$ can take large values when $q$ is close to zero and thus unreliable, \citet{yamada2013relative} proposed the $\beta$-relative density ratio (we slightly abuse $\beta$ to be consistent with our objective): $r_{\beta} = p / (\beta p + (1 - \beta) q)$ for $0 \leq \beta < 1$. The $\beta$-relative $\chi^2$ divergence is then defined as $\chi^2_{\beta}(P \Vert Q) = \frac{1}{2} \mathbb{E}_Q[(r_{\beta} - 1)^2]$. The special cases of our objective would recover $\chi^2(P \Vert Q)$ and $\chi^2_{\beta}(P \Vert Q)$:
\begin{coro}[Fenchel's Dual Program of $\chi^2$ and Relative $\chi^2$] If $\alpha = \beta = 0$ and $\gamma = 1$, our objective recovers $\chi^2 (P \Vert Q)$. If $\alpha = 0$ and $\beta + \gamma = 1$, our objective recovers $\chi^2_{\beta}(P \Vert Q) = \chi^2 (P \Vert \beta P + (1 - \beta) Q)$.
\end{coro}


Very nicely, the $\beta$-relative density ratio is bounded: $\left\|r_{\beta}\right\|_{\infty}=\left\|(\beta+(1-\beta) / r^{-1}\right\|_{\infty}<\frac{1}{\beta} \text { for } \beta>0$ \citep{yamada2013relative}, where $\|\cdot \|_{\infty}$ represents the infinity norm. To illustrate such property, we provide Figure \ref{fig:relative} which demonstrates the behavior of $r_{\beta}$ inspired by \citet{sugiyama2012density}. Here, $r_{\beta}= p / (\beta p + (1 - \beta) q)$ is to estimte the density ratio, where $p\sim\mathcal{N}(0,1)$ and $q\sim\mathcal{N}(0.5, 1)$.  In the figure, the blue dashed line shows the unbounded density ratio could diverge to infinity and potentially lead to unreliable estimation. In contrast, the $\beta$-relative density ratio is successfully bounded by $1/\beta$, as the orange ($\beta=0.5$) and green ($\beta=0.95$) dashed lines shown in the figure. Our method is inspired by the property and further introduces $\alpha$ and $\gamma$ as regularization terms. See \colorbox{yellow}{Appendix} for more details about the bound of our density ratio.

\begin{table}[t!]
    %\hspace{-1.4cm}
    \centering
    \scalebox{0.59}{
    \begin{tabular}{c c c c}
         \toprule
         Objective & \makecell{ Good Training\\Stability} & \makecell{Low Minibatch\\Size Sensitivity} & \makecell{Good Downstream\\Performance} \\
         \midrule \midrule 
          \multicolumn{4}{c}{relating to KL-divergence between $P_{XY}$ and $P_XP_Y$: 
          {\color{red} $J_{\rm DV}$}~\citep{donsker1975asymptotic}, {\color{red}$J_{\rm NWJ}$}~\citep{nguyen2010estimating}, and {\color{red}$J_{\rm CPC}$}~\citep{oord2018representation}} \\ \cmidrule{1-4}
         ${\color{red}J_{\rm DV}(X,Y)}:={\rm sup}_{f\in\mathcal{F}}\,\mathbb{E}_{P_{XY}}[f(x,y)]-\log (\mathbb{E}_{P_XP_Y}[e^{f(x,y)}])$ & \xmark & \cmark & \xmark \\ 
         ${\color{red}J_{\rm NWJ}(X,Y)}:={\rm sup}_{f\in\mathcal{F}}\,\mathbb{E}_{P_{XY}}[f(x,y)]- \mathbb{E}_{P_XP_Y}[e^{f(x,y) - 1}]$ & \xmark & \cmark & \xmark \\
                  ${\color{red}J_{\rm CPC}(X,Y)} := {\rm sup}_{f\in\mathcal{F}}\,\mathbb{E}_{(x, y_1) \sim P_{XY}, \{y_j\}_{j=2}^{N} \sim P_Y} \Big[ \log \big(e^{f(x, y_1)} / \frac{1}{N}\sum_{j=1}^N e^{f(x, y_j)}\big)\Big]$ & \cmark & \xmark & \cmark \\
         \midrule \midrule 
         \multicolumn{4}{c}{relating to JS-divergence between $P_{XY}$ and $P_XP_Y$: {\color{red}$J_{\rm JS}$}~\citep{nowozin2016f}} \\ \cmidrule{1-4}
         ${\color{red}J_{\rm JS}(X,Y)}:={\rm sup}_{f\in\mathcal{F}}\,\mathbb{E}_{P_{XY}}[-\log( 1 + e^{-f(x,y)})]-\mathbb{E}_{P_XP_Y}[\log( 1 + e^{f(x,y)})]$ & \cmark & \cmark & \xmark \\
         \midrule \midrule 
         \multicolumn{4}{c}{relating to Wasserstein-divergence between $P_{XY}$ and $P_XP_Y$: {\color{red}$J_{\rm WPC}$}~\citep{ozair2019wasserstein}, with $\mathcal{F_L}$ denoting the space of 1-Lipschitz functions} \\ \cmidrule{1-4}
         ${\color{red}J_{\rm WPC}(X,Y)}:={\rm sup}_{f\in\mathcal{F_L}}\,\mathbb{E}_{(x, y_1) \sim P_{XY}, \{y_j\}_{j=2}^{N} \sim P_Y} \Big[\log \big( e^{f(x, y_1)} / \frac{1}{N}\sum_{j=1}^N e^{f(x, y_j)}\big)\Big]$ & \cmark & \cmark & \xmark$^\dagger$\\ \midrule \midrule 
         \multicolumn{4}{c}{relating to $\chi^2$-divergence between $P_{XY}$ and $P_XP_Y$: {\color{red}$J_{\rm RPC}$} (ours)} \\ \cmidrule{1-4}
         ${\color{red}J_{\rm RPC}(X,Y)}:={\rm sup}_{f\in\mathcal{F}}\,\mathbb{E}_{P_{XY}}[f(x,y)]-\alpha \mathbb{E}_{P_XP_Y}[f(x,y)]-\frac{\beta}{2} \mathbb{E}_{P_{XY}}\left[f^{2}(x,y)\right]-\frac{\gamma}{2}\mathbb{E}_{P_XP_Y}\left[f^{2}(x,y)\right]$ & \cmark & \cmark & \cmark \\
         \bottomrule
    \end{tabular}
    }
    \caption{\small Different contrastive learning objectives, grouped by measurements of distribution discrepancy. $P_{XY}$ represents the distribution of related samples (positively-paired) and $P_XP_Y$ represents the distribution of unrelated samples (negatively-paired). 
    $f(x, y)\in\mathcal{F}$ for $\mathcal{F}$ being any class of functions $f:\mathcal{X}\times \mathcal{Y}\rightarrow \mathbb{R}$. 
    %$\dagger$: $J_{\rm JSD}$ has better stability than $J_{\rm DV}$ and $J_{\rm NWJ}$ but worse than $J_{\rm CPC}$, $J_{\rm WPC}$ and $J_{\rm RPC}$. 
    $\dagger$: Compared to $J_{\rm CPC}$ and $J_{\rm RPC}$, we empirically find $J_{\rm WPC}$ performs worse on complex real-world image datasets spanning CIFAR-10/-100~\citep{krizhevsky2009learning} and ImageNet~\citep{russakovsky2015imagenet}. 
    }
    \label{tab:objectives}
\end{table}


% \begin{figure}[t!]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[scale=0.27]{fig/gaussian_new.png}
% % \includegraphics[scale=0.27]{fig/alpha_new.png}
% % \includegraphics[scale=0.27]{fig/beta.png}
% % \includegraphics[scale=0.27]{fig/gamma.png}
% \end{center}
% \vspace{-5mm}
% \caption{.}
% \end{figure}
% RPC extends the idea of $\beta$-relative divergence and applied relative parameter to regularize the linear and quadratic score terms of positive samples.  We provide the bound of our density ratio in \colorbox{yellow}{Appendix}. Such design further bounds the variance of our objective.

% Though the third term has a negative coefficient of positive scores, we set $\beta$ to be small so that it serves as a regularizer for scores of positive samples. \colorbox{red}{l2-regularized}

% is a member of the $\textit{f}$-divergences that not only shares similar properties \citep{niu2013squared} with the KL divergence, but also has superior numerical properties \citep{kanamori2013computational} and robustness against outliers \citep{sugiyama2012density}. , and it has been used in semi-supervised representation learning \citep{niu2013squared}. 

==> sections/misc.tex <==
\begin{wraptable}{hrt}{\textwidth}
% \begin{table}[ht]
% \hspace{0.4cm}
% \begin{minipage}[b]{0.4\linewidth}
\small
\centering
\begin{tabular}{c c c c c c c c}
    \toprule
    $\alpha$ & $\beta$ & $\gamma$ & Acc (\%) \\
    \midrule
    0.00 & 0.001 & 1.0 & 78.63\\
    0.00 & 0.002 & 1.0 & 82.50\\
    0.00 & 0.005 & 1.0 & 89.93\\
    0.00 & 0.010 & 1.0 & 88.21\\
    0.00 & 0.001 & 0.75 & 87.00\\
    0.00 & 0.002 & 0.75 & 87.50\\
    0.00 & 0.005 & 0.75 & 76.90\\
    0.00 & 0.01 & 0.75 & 91.20\\
    0.00 & 0.001 & 0.5 & 87.00\\
    0.00 & 0.002 & 0.5 & 87.50\\
    0.00 & 0.005 & 0.5 & 76.90\\
    0.00 & 0.01 & 0.5 & 91.20\\
    \bottomrule
\end{tabular}
% \end{minipage}\hfill
% \end{table}

\end{wraptable}


==> sections/prev_method.tex <==
\section{Method}
Our goal is to present a learning objective that could be more robust to variance and batch size. We start by introducing the general form of our objective, and in the following show how different variants of the objective in vision and speech tasks can be implemented. 


% Another popular discussion about the contrastive objectives is that CPC is upper bounded and would need large batch size to have small estimation bias. To illustrate this point, we write CPC following notations in Equation \ref{eq:RCO_def}:
% % \begin{equation}
% %     I_{CPC} = \,\,\frac{1}{|\sP|}\sum_{(\tilde{\vx_1}, \tilde{\vx_2}) \in \sP}f - \log{(\frac{1}{|\sN|}\, \sum_{(\tilde{\vx_1}, \tilde{\vx_2}) \in \sN}e^f)}
% % \end{equation}
% \begin{equation}
%     I_{CPC} = \,\,\frac{1}{|\sP|}\sum_{(\vx_1, \vx_2) \in \sP}\log{\frac{e^{f(\vx_1, \vx_2)}}{\frac{1}{|\sN'|}\, \sum_{(\tilde{\vx_1}, \tilde{\vx_2}) \in \sN'}e^{f(\tilde{\vx_1}, \tilde{\vx_2})}}}
% \end{equation}
% where $f = f(\tilde{\vx_1}, \tilde{\vx_2})$ is an arbitrary function. For each single positive pair $(\vx_i, \vx_j)$, there are a set of accompanied negative pairs $\sN' \subseteq \sN$. Depending on implementation, $|\sN'|$ could be mutually exclusive or not, but the union of all $|\sN'|$ is $|\sN|$, the set of all negative pairs generated from a batch of samples. the The objective itself cannot exceed $\log{(|\sN|)}$: $I_{CPC} \leq log{(|\sN|)}$ where $|\sN|$ is the size of the negative pair set (need rephrasing and correction here), and we provide the proof in \ref{Appendix:1}. When batch size for evaluating the objective is small, the size of the negative pair set $|\sN|$ will also be small, leading to high bias behaviors (Poole). The intuition is that, CPC is using $softmax$, so that when considering all pairs as an empirical distribution, it assign a probability as high as 1 to the positive pair $(\vx_i, \vx_j)$, by increasing the score of positive pairs $f(\vx_i, \vx_j))$ \textit{relative to} scores of negative pairs. If batch size is small, distinguishing the positive sample by pushing score $f(\vx_i, \vx_j)$ higher would be easier, compared to distinguishing from a large set of negative samples generated by large batch size. This would potentially prevent the objective to learn a more effective representation, as we will show in Section \ref{sec:1}.

==> sections/proofs/proof_props_archive.tex <==
\subsection{Proof of Proposition 1 in the Main Text}
$$
{\hat{J}}_{{\rm RPC}} :=\underset{\theta\in\Theta}{\rm sup}\,\mathbb{E}_{P_{XY}}[f_\theta(x,y)]-\alpha \mathbb{E}_{P_XP_Y}[f_\theta(x,y)]-\frac{\beta}{2} \mathbb{E}_{P_{XY}}\left[f_\theta^{2}(x,y)\right]-\frac{\gamma}{2}\mathbb{E}_{P_XP_Y}\left[f_\theta^{2}(x,y)\right]
$$

\begin{equation*}
\begin{split}
\hat{J}^{m,n}_{\rm RPC} & = \sup_{\theta \in \Theta} \frac{1}{n}\sum_{i=1}^n f_\theta(x_i,y_i) - \alpha \frac{1}{m}\sum_{j=1}^m f_\theta(x'_j,y'_j) - \frac{\beta}{2} \frac{1}{n}\sum_{i=1}^n f_\theta^2(x_i,y_i) - \frac{\gamma}{2} \frac{1}{m}\sum_{j=1}^m f_\theta^2(x'_j,y'_j) \\
& = \sup_{\theta \in \Theta} \hat{J}^{m,n}_{\rm RPC, \theta}
\end{split}
\end{equation*}




\begin{prop}[Boundness of $\hat{J}^{m,n}_{\rm RPC}$] $0 \leq J_{\rm RPC} \leq \frac{1}{2\beta}+\frac{\alpha^2}{2\gamma}$. With high probability, $|J_{\rm RPC} - \hat{J}^{m,n}_{\rm RPC}| \leq  O(n'^{-\frac{1}{2}}),$ where $n' = {\rm min}\,\{n, m\}$. 
\label{prop:RPC_bound2}
\end{prop}


\subsection{Proof of Proposition 2 in the Main Text}
The variance analysis on $\hat{J}^{m,n}_{\rm RPC}$ is from an asymptotic viewpoint. First, leveraging the neural network's universal function approximation~\citep{hornik1989multilayer}, we assume existing a network parameter $\theta^*$ satisfying $f^*(x,y) = f_{\theta^*}(x,y) = r_{\alpha, \beta, \gamma}(x,y)$. Then we recall that $\hat{J}^{m,n}_{\rm RPC}$ is a consistent estimator of ${J}^{\rm RPC}$ (see Proposition~\ref{prop:RPC_bound2}), and under regular conditions, the estimated network parameter $\hat{\theta}$ in $\hat{J}^{m,n}_{\rm RPC}$ satisfying the asymptotic normality in the large sample limit (see Theorem 5.23 in~\citep{van2000asymptotic}). 
%Hence, when $m,n \rightarrow \infty$, $\hat{J}^{m,n}_{\rm RPC, \hat{\theta}} \rightarrow J_{\rm RPC}$ and $\hat{\theta} \rightarrow \theta^*$. Then, 
Let $n' = {\rm min}\{n,m\}$, the asymptotic expansion of $\hat{J}^{m,n}_{\rm RPC}$ has
\begin{equation}
\begin{split}
\hat{J}^{m,n}_{{\rm RPC}, \theta^*} &= \hat{J}^{m,n}_{{\rm RPC}, \hat{\theta}} + \dot{\hat{J}}^{m,n}_{{\rm RPC}, \hat{\theta}}(\theta^* - \hat{\theta}) + o(\| \theta^*  - \hat{\theta}\|) \\
& = \hat{J}^{m,n}_{{\rm RPC}, \hat{\theta}} + \dot{\hat{J}}^{m,n}_{{\rm RPC}, \hat{\theta}}(\theta^* - \hat{\theta}) +  o_p(\frac{1}{\sqrt{n'}}) \\
& = \hat{J}^{m,n}_{{\rm RPC}, \hat{\theta}} +  o_p(\frac{1}{\sqrt{n'}}),
\end{split}
\label{eq:asym1}
\end{equation}
where $ \dot{\hat{J}}^{m,n}_{{\rm RPC}, \hat{\theta}} = 0$ since $\hat{\theta}$ is the estimation from $\hat{J}^{m,n}_{{\rm RPC}} = \underset{f_\theta \in \mathcal{F}_\Theta}{\rm sup}\,\hat{J}^{m,n}_{{\rm RPC}, \theta}$. 

Next, we define 
$$\mathbb{E}[\hat{J}_{\rm RPC, \hat{\theta}}] = \mathbb{E}_{P_{XY}} [f_{\hat{\theta}}(x,y)] - \alpha \mathbb{E}_{P_XP_Y} [f_{\hat{\theta}}(x,y)] - \frac{\beta}{2}\mathbb{E}_{P_{XY}} [ f_{\hat{\theta}}^2(x,y)] - \frac{\gamma}{2} \mathbb{E}_{P_XP_Y} [f_{\hat{\theta}}^2(x,y)].$$
Likewise, the asymptotic expansion of $\mathbb{E}[\hat{J}_{\rm RPC, \theta}]$ has
\begin{equation}
\begin{split}
    \mathbb{E}[\hat{J}_{\rm RPC, \hat{\theta}}] &= \mathbb{E}[\hat{J}_{\rm RPC, \theta^*}] + \mathbb{E}[\dot{\hat{J}}_{\rm RPC, \theta^*}](\hat{\theta} - \theta^*) + o(\| \hat{\theta} - \theta^* \|) \\
    & = \mathbb{E}[\hat{J}_{\rm RPC, \theta^*}] + \mathbb{E}[\dot{\hat{J}}_{\rm RPC, \theta^*}](\hat{\theta} - \theta^*) + o_p(\frac{1}{\sqrt{n'}}) \\
    & = \mathbb{E}[\hat{J}_{\rm RPC, \theta^*}] + o_p(\frac{1}{\sqrt{n'}}),
\end{split}
\label{eq:asym2}
\end{equation}
where $\mathbb{E}[\dot{\hat{J}}_{\rm RPC, \theta^*}] = 0$ since $\mathbb{E}[\hat{J}_{\rm RPC, \theta^*}] = J_{\rm RPC}$ and $\theta^*$ satisfying $f^*(x,y)=f_{\theta^*}(x,y)$.

Combining equations~\ref{eq:asym1} and~\ref{eq:asym2}:
\begin{equation*}
\begin{split}
    \hat{J}^{m,n}_{{\rm RPC}, \hat{\theta}} - \mathbb{E}[\hat{J}_{\rm RPC, \hat{\theta}}]= & \hat{J}^{m,n}_{{\rm RPC}, \theta^*} - J_{\rm RPC} +  o_p(\frac{1}{\sqrt{n'}}) \\
    = & \frac{1}{n}\sum_{i=1}^n f_\theta^*(x_i,y_i) - \alpha \frac{1}{m}\sum_{j=1}^m f_\theta^*(x'_j,y'_j) - \frac{\beta}{2} \frac{1}{n}\sum_{i=1}^n f_{\theta^*}^2(x_i,y_i) - \frac{\gamma}{2} \frac{1}{m}\sum_{j=1}^m f_{\theta^*}^2(x'_j,y'_j) \\
    & - \mathbb{E}_{P_{XY}}[f^*(x,y)]+\alpha \mathbb{E}_{P_XP_Y}[f^*(x,y)]+\frac{\beta}{2} \mathbb{E}_{P_{XY}}\left[{f^*}^2(x,y)\right]+\frac{\gamma}{2}\mathbb{E}_{P_XP_Y}\left[{f^*}^2(x,y)\right] +  o_p(\frac{1}{\sqrt{n'}}) \\
    = & \frac{1}{n}\sum_{i=1}^n r_{\alpha, \beta, \gamma}(x_i,y_i) - \alpha \frac{1}{m}\sum_{j=1}^m r_{\alpha, \beta, \gamma}(x'_j,y'_j) - \frac{\beta}{2} \frac{1}{n}\sum_{i=1}^n r_{\alpha, \beta, \gamma}^2(x_i,y_i) - \frac{\gamma}{2} \frac{1}{m}\sum_{j=1}^m r_{\alpha, \beta, \gamma}^2(x'_j,y'_j)  \\
    & - \mathbb{E}_{P_{XY}}[r_{\alpha, \beta, \gamma}(x,y)]+\alpha \mathbb{E}_{P_XP_Y}[r_{\alpha, \beta, \gamma}(x,y)]+\frac{\beta}{2} \mathbb{E}_{P_{XY}}\left[r_{\alpha, \beta, \gamma}^2(x,y)\right]+\frac{\gamma}{2}\mathbb{E}_{P_XP_Y}\left[r_{\alpha, \beta, \gamma}^2(x,y)\right] \\
    & +  o_p(\frac{1}{\sqrt{n'}}) \\
    = & \Bigg(\frac{1}{n} \sum_{i=1}^n  r_{\alpha, \beta, \gamma}(x_i,y_i) - \frac{\beta}{2}r_{\alpha, \beta, \gamma}^2(x_i,y_i) -\mathbb{E}_{P_{XY}}\bigg[r_{\alpha, \beta, \gamma}(x,y) - \frac{\beta}{2}r_{\alpha, \beta, \gamma}^2(x,y)\bigg] \Bigg) \\
    & - \Bigg( \frac{1}{m} \sum_{j=1}^m \alpha r_{\alpha, \beta, \gamma}(x'_j,y'_j) + \frac{\gamma}{2}r^2_{\alpha, \beta, \gamma}(x'_j,y'_j) - \mathbb{E}_{P_XP_Y}\bigg[\alpha r_{\alpha, \beta, \gamma}(x,y) + \frac{\gamma}{2}r^2_{\alpha, \beta, \gamma}(x,y)\bigg] \Bigg)\\
    & + o_p(\frac{1}{\sqrt{n'}}).
\end{split}
\end{equation*}
Therefore, the asymptotic Variance of $\hat{J}^{m,n}_{{\rm RPC}}$ is
\begin{equation*}
\begin{split}
    \Var [\hat{J}^{m,n}_{{\rm RPC}}] = \frac{1}{n} \Var_{P_{XY}} [r_{\alpha, \beta, \gamma}(x,y) - \frac{\beta}{2} r^2_{\alpha, \beta, \gamma}(x,y)] + \frac{1}{m} \Var_{P_XP_Y} [\alpha r_{\alpha, \beta, \gamma}(x,y) +  \frac{\gamma}{2} r^2_{\alpha, \beta, \gamma}(x,y)] + o(\frac{1}{n'}). 
\end{split}
\end{equation*}

First, we look at $\Var_{P_{XY}} [r_{\alpha, \beta, \gamma}(x,y) - \frac{\beta}{2} r^2_{\alpha, \beta, \gamma}(x,y)]$. Since $\beta > 0$ and $-\frac{\alpha}{\gamma}\leq r_{\alpha, \beta, \gamma} \leq \frac{1}{\beta}$, simple calculation gives us $
-\frac{2\alpha \gamma + \beta \alpha^2}{2 \gamma^2}\leq r_{\alpha, \beta, \gamma}(x,y) - \frac{\beta}{2} r^2_{\alpha, \beta, \gamma}(x,y) \leq \frac{1}{2\beta}$. Hence, 
$$
\Var_{P_{XY}} [r_{\alpha, \beta, \gamma}(x,y) - \frac{\beta}{2} r^2_{\alpha, \beta, \gamma}(x,y)] \leq {\rm max}\bigg\{\Big(\frac{2\alpha \gamma + \beta \alpha^2}{2 \gamma^2}\Big)^2, \Big(\frac{1}{2\beta}\Big)^2\bigg\}.
$$
Next, we look at $\Var_{P_XP_Y} [\alpha r_{\alpha, \beta, \gamma}(x,y) +  \frac{\gamma}{2} r^2_{\alpha, \beta, \gamma}(x,y)]$. Since $\alpha \geq 0, \gamma > 0$ and $-\frac{\alpha}{\gamma}\leq r_{\alpha, \beta, \gamma} \leq \frac{1}{\beta}$,
simple calculation gives us $
-\frac{\alpha^2}{2 \gamma}\leq \alpha r_{\alpha, \beta, \gamma}(x,y) +  \frac{\gamma}{2} r^2_{\alpha, \beta, \gamma}(x,y) \leq \frac{2\alpha \beta + \gamma}{2\beta^2}$. Hence, 
$$
\Var_{P_XP_Y} [\alpha r_{\alpha, \beta, \gamma}(x,y) +  \frac{\gamma}{2} r^2_{\alpha, \beta, \gamma}(x,y)] \leq {\rm max}\bigg\{\Big(\frac{\alpha^2 }{2 \gamma}\Big)^2, \Big( \frac{2\alpha \beta + \gamma}{2\beta^2} \Big)^2\bigg\}.$$
Combining everything together,  we restate the Proposition 2 in the main text:
\begin{prop}[Asymptotic Variance of $\hat{J}^{m,n}_{\rm RPC}$] \label{prop:variance} 
$$\Var [\hat{J}^{m,n}_{{\rm RPC}}] \leq \frac{1}{n} {\rm max}\bigg\{\Big(\frac{2\alpha \gamma + \beta \alpha^2}{2 \gamma^2}\Big)^2, \Big(\frac{1}{2\beta}\Big)^2\bigg\} + \frac{1}{m} {\rm max}\bigg\{\Big(\frac{\alpha^2 }{2 \gamma}\Big)^2, \Big( \frac{2\alpha \beta + \gamma}{2\beta^2} \Big)^2\bigg\} + o(\frac{1}{n'}).
$$
\label{prop:var2}
\end{prop}
